Dynamic Refinement Network for Oriented and Densely Packed Object Detection

Object detection has achieved remarkable progress in the past decade. However, the detection of oriented and densely packed objects remains challenging because of following inherent reasons: (1) receptive fields of neurons are all axis-aligned and of the same shape, whereas objects are usually of diverse shapes and align along various directions; (2) detection models are typically trained with generic knowledge and may not generalize well to handle specific objects at test time; (3) the limited dataset hinders the development on this task. To resolve the first two issues, we present a dynamic refinement network that consists of two novel components, i.e., a feature selection module (FSM) and a dynamic refinement head (DRH). Our FSM enables neurons to adjust receptive fields in accordance with the shapes and orientations of target objects, whereas the DRH empowers our model to refine the prediction dynamically in an object-aware manner. To address the limited availability of related benchmarks, we collect an extensive and fully annotated dataset, namely, SKU110K-R, which is relabeled with oriented bounding boxes based on SKU110K. We perform quantitative evaluations on several publicly available benchmarks including DOTA, HRSC2016, SKU110K, and our own SKU110K-R dataset. Experimental results show that our method achieves consistent and substantial gains compared with baseline approaches. The code and dataset are available at https://github.com/Anymake/DRN_CVPR2020.

==> figs/att_map.tex <==
\begin{figure*}[!htb]
\centering
\subfigure[]{
\includegraphics[width=0.49\linewidth]{images/att/P0007__1__0___824__att.png}}
\subfigure[]{
\includegraphics[width=0.49\linewidth]{images/att/P0060__1__1648___1229__att.png}}
\caption{Illustrations of attention maps in FSM.}
\label{fig:att_map}
\end{figure*}

==> figs/fig_att.tex <==
\begin{figure}[h]
\centering
\subfigure[Before rotation]{
\includegraphics[width=0.47\linewidth, trim=0px 50px 0px 30px, clip]{images/att/att_af0.pdf}
\label{fig:att_af_reb}}
\subfigure[After rotation]{
\includegraphics[width=0.47\linewidth, trim=0px 50px 0px 30px, clip]{images/att/att_bf0.pdf}
\label{fig:att_bf_reb}}
\caption{Illustrations of dynamic refinement on classification (a) and regression (b).
%An illustration of classification and regression task.
Each solid dot represents one sample. 
With the general knowledge learned in the training procedure, classifier and regressor make predictions suffering from the lack of flexibility. Model should changes over samples. The arrows show the promising refinements for better performance.}
\label{fig:att}
\end{figure}


==> figs/fig_att_reb.tex <==
\begin{figure}[h]
\centering
\subfigure[Before rotation]{
\includegraphics[width=0.47\linewidth, trim=0px 50px 0px 30px, clip]{images/att/att_af0.pdf}
\label{fig:att_af_reb}}
\subfigure[After rotation]{
\includegraphics[width=0.47\linewidth, trim=0px 50px 0px 30px, clip]{images/att/att_bf0.pdf}
\label{fig:att_bf_reb}}
% \caption{Illustrations of dynamic refinement on classification (a) and regression (b).
% %An illustration of classification and regression task.
% Each solid dot represent a sample. 
% With the general knowledge learned in training procedure, classifier and regressor make predictions suffering from the lack of flexibility. Model should changes over samples. The arrows show the promising refinements for better performance.}
\label{fig:att_reb}
\end{figure}

==> figs/fig_centernet-r_baseline.tex <==
\begin{figure*}%[!htb]
\centering
\includegraphics[width=\linewidth]{images/centernet_r.png}
\caption{The overall framework of CenterNet$^\dagger$. We insert deformable center pooling layer between backbone and heads. }
\label{fig:ctr_baseline}
\end{figure*}

==> figs/fig_rosku_sta.tex <==
\begin{figure}[!htb]
\centering
\subfigure[SKU110K]{
\includegraphics[width=0.95\linewidth]{images/rosku/sku110k.png}
\label{fig:sku_sta}}
\subfigure[SKU110K-R]{
\includegraphics[width=0.9\linewidth]{images/rosku/sku110k-r.png}
\label{fig:rsku_sta}}
\caption{Statistics of orientation distribution of SKU110K and SKU110K-R. Y axis represents the number of instance and X axis represents the orientation angle.}
\label{fig:rosku_sta}
\end{figure}

==> figs/fig_vis_rsku.tex <==
% \begin{figure*}%[!htb]
% \setcounter{subfigure}{0}
% 	\centering
% 	\subfigure{
% 		\includegraphics[height=0.28\linewidth]{images/rosku/sku_h0_cps.jpg}}
% 	\subfigure{
% 		\includegraphics[height=0.28\linewidth]{images/rosku/sku_h1_cps.jpg}}
% 	\subfigure{
% 		\includegraphics[height=0.28\linewidth]{images/rosku/sku_h2_cps.jpg}}
% 	\subfigure{
% 		\includegraphics[height=0.28\linewidth]{images/rosku/sku_h3_cps.jpg}}
% 	\subfigure{
% 		\includegraphics[height=0.28\linewidth]{images/rosku/sku_r0_cps.jpg}}
% 	\subfigure{
% 		\includegraphics[height=0.28\linewidth]{images/rosku/sku_r1_cps.jpg}}
% 	\subfigure{
% 		\includegraphics[height=0.28\linewidth]{images/rosku/sku_r2_cps.jpg}}
% 	\subfigure{
% 		\includegraphics[height=0.28\linewidth]{images/rosku/sku_r3_cps.jpg}}
% % 	\subfigure[Ours]{
% % 		\includegraphics[width=0.23\linewidth]{images/sanfan/OurCollage_HTS}}
% 	\caption{Examples of images in SKU110K.}
% 	\label{fig:vis_rsku}
% \end{figure*}

\begin{figure*}[!htb]
\setcounter{subfigure}{0}
	\centering
	\subfigure{
		\includegraphics[width=0.24\linewidth]{images/rosku/sku_h0_cps.jpg}}
	\subfigure{
		\includegraphics[width=0.24\linewidth]{images/rosku/sku_h1_cps.jpg}}
	\subfigure{
		\includegraphics[width=0.24\linewidth]{images/rosku/sku_h2_cps.jpg}}
	\subfigure{
		\includegraphics[width=0.24\linewidth]{images/rosku/sku_h3_cps.jpg}}
	\subfigure{
		\includegraphics[width=0.24\linewidth]{images/rosku/sku_r0_cps.jpg}}
	\subfigure{
		\includegraphics[width=0.24\linewidth]{images/rosku/sku_r1_cps.jpg}}
	\subfigure{
		\includegraphics[width=0.24\linewidth]{images/rosku/sku_r2_cps.jpg}}
	\subfigure{
		\includegraphics[width=0.24\linewidth]{images/rosku/sku_r3_cps.jpg}}
% 	\subfigure[Ours]{
% 		\includegraphics[width=0.23\linewidth]{images/sanfan/OurCollage_HTS}}
	\caption{Some sample images from SKU110K. The images in \textbf{top} row are annotated with horizontal bounding boxes while the images in \textbf{bottom} row are with oriented bounding boxes.}
	\label{fig:vis_rsku}
\end{figure*}

==> tabs/dota_main_bak.tex <==
\begin{table*}%[!ht]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lccccccccccccccccc}
\toprule
Method &  PL &  BD &  BR &  GTF &  SV &  LV &  SH &  TC &  BC &  ST &  SBF &  RA &  HA &  SP &  HC &  mAP\\ \hline\hline
\textbf{OBB}& \\
\hline
SSD~\cite{Liu:2016:SSD} & 39.83 & 9.09 & 0.64 & 13.18 & 0.26 & 0.39 & 1.11 & 16.24 & 27.57 & 9.23 & 27.16 & 9.09 & 3.03 & 1.05 & 1.01 & 10.59 \\

YOLOv2~\cite{Redmon:2017:Yolo9000} & 39.57 & 20.29 & 36.58 & 23.42 & 8.85 & 2.09 & 4.82 & 44.34 & 38.35 & 34.65 & 16.02 & 37.62 & 47.23 & 25.5 & 7.45 & 21.39 \\

FR-O~\cite{xia2018dota} & 79.42 & 44.13 & 17.7 & 64.05 & 35.3 & 38.02 & 37.16 & 89.41 & 69.64 & 59.28 & 50.3 & 52.91 & 47.89 & 47.4 & 46.3 & 54.13 \\

ICN~\cite{azimi2018towards}  & 81.40 & 74.30 & 47.70 & 70.30 & 64.90 & 67.80 & 70.00 & 90.80 & 79.10 & 78.20 & 53.60 & 62.90 & 67.00 & 64.20 & 50.20 & 68.20 \\

R-DFPN~\cite{yang2018automatic} & 80.92 & 65.82 & 33.77 & 58.94 & 55.77 & 50.94 & 54.78 & 90.33 & 66.34 & 68.66 & 48.73 & 51.76 & 55.10 & 51.32 & 35.88 & 57.94 \\

R$^2$CNN~\cite{jiang2017r2cnn} & 80.94 & 65.67 & 35.34 & 67.44 & 59.92 & 50.91 & 55.81 & 90.67 & 66.92 & 72.39 & 55.06 & 52.23 & 55.14 & 53.35 & 48.22 & 60.67 \\

RRPN~\cite{ma2018arbitrary} & 88.52 & 71.20 & 31.66 & 59.30 & 51.85 & 56.19 & 57.25 & 90.81 & 72.84 & 67.38 & 56.69 & 52.84 & 53.08 & 51.94 & 53.58 & 61.01 \\

RoI-Transformer~\cite{ding2019learning} & 88.64 & 78.52 & 43.44 & {\bf 75.92} & {\bf 68.81} & {\bf 73.68} & 83.59 & 90.74 & 77.27 & 81.46 & {\bf58.39} & 53.54 & {\bf62.83} & 58.93 & 47.67 & 69.56 \\

SCRDet~\cite{yang2019scrdet}  & 89.98 & 80.65 & 52.09 & 68.36 & 68.36 &  60.32 & 72.41 & 90.85 & 87.94 & 86.86 & {\bf65.02} & 66.68 & 66.25 & 68.24 & 65.21 & 72.61 \\
\hline
baseline & 89.41 & 78.88 & 43.55 & 61.24 & 66.49 & 70.20 & {\bf85.52} & 90.79 & 85.19 & 82.91 & 56.92 & 56.81 & 61.35 & 67.25 & 51.05 & 69.84\\
+FSM & 89.41 & 78.88 & 43.55 & 61.24 & 66.49 & 70.20 & {\bf85.52} & 90.79 & 85.19 & 82.91 & 56.92 & 56.81 & 61.35 & 67.25 & 51.05 & 69.84\\
+DRH & 89.41 & 78.88 & 43.55 & 61.24 & 66.49 & 70.20 & {\bf85.52} & 90.79 & 85.19 & 82.91 & 56.92 & 56.81 & 61.35 & 67.25 & 51.05 & 69.84\\
DRN (our) & {\bf89.41} & {\bf78.88} & {\bf43.55} & 61.24 & 66.49 & 70.20 & {\bf85.52} & {\bf90.79} & {\bf85.19} & {\bf82.91} & 56.92 & {\bf56.81} & 61.35 & {\bf67.25} & {\bf51.05} & {\bf69.84}\\
DRN$^*$ (our) & {\bf89.41} & {\bf78.88} & {\bf43.55} & 61.24 & 66.49 & 70.20 & {\bf85.52} & {\bf90.79} & {\bf85.19} & {\bf82.91} & 56.92 & {\bf56.81} & 61.35 & {\bf67.25} & {\bf51.05} & {\bf69.84}\\
DRN$^**$ (our) & {\bf89.41} & {\bf78.88} & {\bf43.55} & 61.24 & 66.49 & 70.20 & {\bf85.52} & {\bf90.79} & {\bf85.19} & {\bf82.91} & 56.92 & {\bf56.81} & 61.35 & {\bf67.25} & {\bf51.05} & {\bf69.84}\\
\hline
\textbf{HBB} \\ \hline

SSD ~\cite{Liu:2016:SSD} & 44.74 & 11.21 & 6.22 & 6.91 & 2.00 & 10.24 & 11.34 & 15.59 & 12.56 & 17.94 & 14.73 & 4.55 & 4.55 & 0.53 & 1.01 & 10.94 \\

YOLOv~\cite{Redmon:2017:Yolo9000} & 76.90 & 33.87 & 22.73 & 34.88 & 38.73 & 32.02 & 52.37 & 61.65 & 48.54 & 33.91 & 29.27 & 36.83 & 36.44 & 38.26 & 11.61 & 39.20 \\

R-FCN~\cite{dai2016r} & 79.33 & 44.26 & 36.58 & 53.53  & 39.38 & 34.15  & 47.29 & 45.66 & 47.74 & 65.84 & 37.92 & 44.23 & 47.23 & 50.64 & 34.90 & 47.24 \\

FR-H~\cite{ren2015faster} & 80.32 & 77.55 & 32.86 & 68.13 & 53.66 & 52.49 & 50.04 & 90.41 & 75.05 & 59.59 & 57.00 & 49.81 & 61.69 & 56.46 & 41.85 & 60.46 \\

FPN~\cite{lin2017feature} & 88.70 & 75.10 & 52.60 & 59.20 & 69.40 & 78.80 & 84.50 & 90.60 & 81.30 & 82.60 & 52.50 & 62.10 & 76.60 & 66.30 & 60.10 & 72.00 \\

ICN~\cite{azimi2018towards} & 90.00 & 77.70 & 53.40 & 73.30 & 73.50 & 65.00 & 78.20 & 90.80 & 79.10 & 84.80 & 57.20 & 62.10 & 73.50 & 70.20 & 58.10 & 72.50 \\

SCRDet~\cite{yang2019scrdet}  & 90.18 & 81.88 & 55.30 & {\bf 73.29} & {\bf 72.09} & {\bf 77.65} & 78.06 & 90.91 & 82.44 & 86.39 & {\bf64.53} & 63.45 & {\bf75.77} & 78.21 & 60.11 & 75.35 \\

\hline

baseline & {\bf89.41} & {\bf78.88} & {\bf43.55} & 61.24 & 66.49 & 70.20 & {\bf85.52} & {\bf90.79} & {\bf85.19} & {\bf82.91} & 56.92 & {\bf56.81} & 61.35 & {\bf67.25} & {\bf51.05} & {\bf69.84}\\

DRN (our) & {\bf89.41} & {\bf78.88} & {\bf43.55} & 61.24 & 66.49 & 70.20 & {\bf85.52} & {\bf90.79} & {\bf85.19} & {\bf82.91} & 56.92 & {\bf56.81} & 61.35 & {\bf67.25} & {\bf51.05} & {\bf69.84}\\

\hline

\bottomrule
\end{tabular}}
\caption{Evaluation results of OBB and HBB task on DOTA dataset. The category names are abbreviated: PL-PLane, BD-Baseball Diamond, BR-BRidge, GTF-Ground Field Track, SV-Small Vehicle, LV-Large Vehicle, SH-SHip, TC-Tennis Court, BC-Basketball Court, ST-Storage Tank, SBF-Soccer-Ball Field, RA-RoundAbout, HA-Harbor, SF-Swimming Pool, and HC-HeliCopter. }
\label{tab:OBB_HBB}
\end{table*}

==> tabs/dota_main_sup.tex <==
\begin{table*}[!ht]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lccccccccccccccccc}
\toprule
Method &  PL &  BD &  BR &  GTF &  SV &  LV &  SH &  TC &  BC &  ST &  SBF &  RA &  HA &  SP &  HC &  mAP\\ \hline
\textbf{one-stage method} \\ \hline
SSD [25] & 39.83 & 9.09 & 0.64 & 13.18 & 0.26 & 0.39 & 1.11 & 16.24 & 27.57 & 9.23 & 27.16 & 9.09 & 3.03 & 1.05 & 1.01 & 10.59 \\

YOLOv2 [31] & 39.57 & 20.29 & 36.58 & 23.42 & 8.85 & 2.09 & 4.82 & 44.34 & 38.35 & 34.65 & 16.02 & 37.62 & 47.23 & 25.5 & 7.45 & 21.39 \\

FR-O [37] & 79.42 & 44.13 & 17.7 & 64.05 & 35.3 & 38.02 & 37.16 & 89.41 & 69.64 & 59.28 & 50.3 & 52.91 & 47.89 & 47.4 & 46.3 & 54.13 \\ \hline
\textbf{two-stage method} \\ \hline
ICN [1]  & 81.40 & 74.30 & 47.70 & 70.30 & 64.90 & 67.80 & 70.00 & 90.80 & 79.10 & 78.20 & 53.60 & 62.90 & 67.00 & 64.20 & 50.20 & 68.20 \\

R-DFPN [38] & 80.92 & 65.82 & 33.77 & 58.94 & 55.77 & 50.94 & 54.78 & 90.33 & 66.34 & 68.66 & 48.73 & 51.76 & 55.10 & 51.32 & 35.88 & 57.94 \\

R$^2$CNN [14] & 80.94 & 65.67 & 35.34 & 67.44 & 59.92 & 50.91 & 55.81 & 90.67 & 66.92 & 72.39 & 55.06 & 52.23 & 55.14 & 53.35 & 48.22 & 60.67 \\

RRPN [28] & 88.52 & 71.20 & 31.66 & 59.30 & 51.85 & 56.19 & 57.25 & 90.81 & 72.84 & 67.38 & 56.69 & 52.84 & 53.08 & 51.94 & 53.58 & 61.01 \\

RoI-Transformer$^{**}$[3] & 88.64 & 78.52 & 43.44 &  {\bf75.92} & 68.81 &  73.6 & 83.59 & 90.74 & 77.27 & 81.46 & 58.39 & 53.54 & 62.83 & 58.93 & 47.67 & 69.56 \\

SCRDet$^{**}$ [39]  & \textbf{89.98} & 80.65 & \textbf{52.09} & 68.36 & 68.36 &  60.32 & 72.41 & {\bf90.85} & {\bf87.94} & {\bf86.86} &{\bf65.02} & {\bf66.68} & 66.25 & 68.24 & \textbf{65.21} & 72.61 \\
\hline
\textbf{anchor-free method} \\ \hline
baseline~[41] & 89.02 & 69.71 & 37.62 & 63.42 & 65.23 & 63.74 & 77.28 & 90.51 & 79.24 & 77.93 & 44.83 & 54.64 & 55.93 & 61.11 & 45.71 & 65.04\\
baseline$^{**}$~[41] & 89.56 & 79.83 & 43.8 & 66.54 & 65.58 & 66.09 & 83.11 & 90.72 & 83.72 & 84.3 & 55.62 & 58.71 & 62.48 & 68.33 & 50.77 & 69.95\\
% +FSM & 89.41 & 78.88 & 43.55 & 61.24 & 66.49 & 70.20 & {\bf85.52} & 90.79 & 85.19 & 82.91 & 56.92 & 56.81 & 61.35 & 67.25 & 51.05 & 69.84\\
% +DRH & 89.41 & 78.88 & 43.55 & 61.24 & 66.49 & 70.20 & {\bf85.52} & 90.79 & 85.19 & 82.91 & 56.92 & 56.81 & 61.35 & 67.25 & 51.05 & 69.84\\
DRN (Ours) & 88.91 & 80.222 & 43.52 & 63.35 & 73.48 & 70.69 & 84.94 & 90.14 & 83.85 & 84.11 & 50.12 & 58.41 & 67.62 & 68.60 & 52.50 & 70.70\\
DRN$^*$ (Ours) & 88.98 & 81.96 & 47.22 & 64.10 & 69.35 & 63.53 & 83.99 & 90.57 & 83.69 & 84.89 & 51.53 & 60.39 & 69.30 &69.63 & 58.48 & 71.17\\
DRN$^{**}$ (Ours) & 89.71 & {\bf82.34} & 47.22 & 64.10 & \textbf{76.22} & \textbf{74.43} & {\bf85.84} & 90.57 & 86.18 & 84.89 & 57.65 & 61.93 & {\bf69.30} & {\bf69.63} & 58.48 & {\bf73.23}\\
% DRN$^{**}$ (Ours)  &\multicolumn{16}{c}{\textbf{Please see results in supplementary}}.\\
\hline
\bottomrule
\end{tabular}}
\caption{Evaluation results of OBB task on DOTA dataset. The category names are abbreviated: PL-PLane, BD-Baseball Diamond, BR-BRidge, GTF-Ground Field Track, SV-Small Vehicle, LV-Large Vehicle, SH-SHip, TC-Tennis Court, BC-Basketball Court, ST-Storage Tank, SBF-Soccer-Ball Field, RA-RoundAbout, HA-Harbor, SF-Swimming Pool, and HC-HeliCopter. $(\cdot)^{*}$ represents testing with flip and $(\cdot)^{**}$ represents testing with both flip and multi-scale. The other results of ours are all without any test augmentation.}
\label{tab:dota_main_sup}
\end{table*}

==> tabs/fsm_abl_reb.tex <==
\begin{table}[h]
\small
\centering
% \resizebox{.45\textwidth}{!}{
\begin{tabular}{lcccc}
	\toprule
      Method &MK &DCN & AP$_{50}$ & AP$_{75}$  \\ \hline
      Baseline & & &  63.4 & 34.6 \\ \hline
     \multirow{3}{*}{FSM}
      & $33$ &$\checkmark$  & 63.5 & 34.8 \\
      & $33,13$ &$\checkmark$  & 63.6 &34.9 \\
      & $33,13,31$ &$\checkmark$ &63.9 & 35.2 \\
	\bottomrule
\end{tabular}
% }
% \caption{Ablation studies about FSM on DOTA validation set. MK represents the multiple kernels using in FSM. $33,13,31$ represents the kernel size $(3,3), (1,3)$ and $(3,1)$, respectively. DCN and ROT represents whether to use the Deformable Convolution Layer and Rotation Convolution Layer.}
\label{tab:fsm_reb}
\end{table}

